Online Partial Service Hosting at the Edge

We consider the problem of service hosting where an application provider can dynamically rent edge computing resources and serve user requests from the edge to deliver a better quality of service. A key novelty of this work is that we allow the service to be hosted partially at the edge which enables a fraction of the user query to be served by the edge. We model the total cost for (partially) hosting a service at the edge as a combination of the latency in serving requests, the bandwidth consumption, and the time-varying cost for renting edge resources. We propose an online policy called $\alpha$-RetroRenting ($\alpha$-RR) which dynamically determines the fraction of the service to be hosted at the edge in any time-slot, based on the history of the request arrivals and the rent cost sequence. As our main result, we derive an upper bound on $\alpha$-RR's competitive ratio with respect to the offline optimal policy that knows the entire request arrival and rent cost sequence in advance. We conduct extensive numerical evaluations to compare the performance of $\alpha$-RR with various benchmarks for synthetic and trace-based request arrival and rent cost processes, and find several parameter regimes where $\alpha$-RR's ability to store the service partially greatly improves cost-efficiency.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> proof_outlines.tex <==
\subsection{Proof Outline for Theorem \ref{thm:RR_adv}}
We divide time into frames such that Frame $i$ for $i \in \mathbb{Z}^+$ starts when OPT-OFF downloads the service for the $i^{\text{th}}$ time. We refer to the time interval before the beginning of the first frame as Frame 0. Note that by definition, in all frames, except maybe the last frame, there is exactly one eviction by OPT-OFF.

\begin{figure}[ht]
	\centering
	\begin{tikzpicture}
	\foreach \x in {0,0.3,0.6,...,7.2}{
		\draw[] (\x,0) --  (\x+0.3,0);
		\draw[gray] (\x,-1mm) -- (\x,1mm);
	}
	
	\draw[<->,color=black] (0.25,14mm) -- 
	node[above=0mm,pos=0.5]{$i.a$} (2.35,14mm);
	\draw[<->,color=black] (2.35,14mm) -- 
	node[above=0mm,pos=0.5]{$i.b$} (4.15,14mm);
	\draw[<->,color=black] (4.15,14mm) -- 
	node[above=0mm,pos=0.5]{$i.c$} (5.65,14mm);
	\draw[<->,color=black] (5.65,14mm) -- 
	node[above=0mm,pos=0.5]{$i.d$} (6.85,14mm);
	
	\foreach \x in {0.25,2.35,4.15,5.65,6.85}{
		\draw[gray] (\x,12mm) -- (\x,16mm);
	}
	\draw[gray] (7.2,-1mm) -- (7.2,1mm);
	\draw[-latex] (0.25,10mm) -- node[above=5mm]{} (0.25,0mm);
	\draw[-latex] (6.85,10mm) -- node[above=5mm]{} (6.85,0mm);
	\draw[-latex] (4.15,0mm) -- node[above=5mm]{} (4.15,10mm);
	\draw[-latex,color=red] (2.35,10mm) -- node[above=5mm]{} (2.35,0mm);
	\draw[-latex,color=red] (5.65,0mm) -- node[above=5mm]{} (5.65,10mm);
	
	\draw[<->,color=black] (0.3,-2mm) -- node[below=0mm,pos=0.5]{Frame 
		$i$} (6.9,-2mm);
	
	\draw[black] (0.3,-1mm) -- (0.3,-3mm);
	\draw[black] (6.9,-1mm) -- (6.9,-3mm);
	
	\node[] at (7.65,-0.85) {OPT-OFF};
	
	\filldraw[fill=black!] (0.25,-1) rectangle (4.15,-0.7);
	\filldraw[fill=white!40] (4.15,-1) rectangle (6.85,-0.7);
	\node[] at (7.25,-1.4) {RR};
	\filldraw[fill=white!40] (0.25,-1.5) rectangle (2.4,-1.2);
	\filldraw[fill=red!] (2.4,-1.5) rectangle (5.7,-1.2);
	\filldraw[fill=white!40] (5.7,-1.5) rectangle (6.85,-1.2);
	
	
	\end{tikzpicture}
	\caption{Illustration showing 
	download and eviction by OPT-OFF and  RR in the $i^{\text{th}}$ frame. 
	Downward arrows represent fetches, upward arrows indicate evictions. 
	Black and red arrows correspond to the OPT-OFF and RR policy respectively. 
	The two bars below the time-line indicate the state of the system under 
	OPT-OFF and  RR. The solid black and solid red portions represent the 
	intervals during with OPT-OFF and RR host  the service respectively.}
	%\vspace*{-10pts}
\label{fig:OPT-OFF_RR_frame_proofoutline}
\end{figure}

We use the properties of RR and OPT-OFF to show that each frame in which OPT-OFF evicts the service has the following structure (Figure \ref{fig:OPT-OFF_RR_frame_proofoutline}):
\begin{enumerate}
	\item[--] RR fetches and evicts the service exactly once each. 
	\item[--] RR does not host  the service at the beginning of the frame.
    \item[--] The fetch by RR in Frame $i$ is before OPT-OFF evicts the service in Frame $i$.
    \item[--] The eviction by RR in Frame $i$ is after OPT-OFF evicts the service in Frame $i$.
\end{enumerate}
We note that both RR and OPT-OFF fetch exactly once in a frame and therefore, the fetch cost under RR and OPT-OFF is identical for both policies. 

We divide Frame $i$ into four sub-frames defined as follows. 
\begin{enumerate}
	\item[--] $i.a$: OPT-OFF hosts  the service, while RR does not.
    \item[--] $i.b$: OPT-OFF and RR both host  the service.
    \item[--] $i.c$: OPT-OFF does not host  the service while RR does.
    \item[--] $i.d$: OPT-OFF and RR both don't host  the service. 
\end{enumerate}

The service and rent costs are identical for OPT-OFF and RR in Sub-frame $i.b$ and Sub-frame $i.d$. 

We show that the difference between the service and rent costs incurred by RR and OPT-OFF in Sub-frame $i.a$ and Sub-frame $i.c$ is upper bounded by $M+\kappa-c_{\text{min}}$ and $M+c_{\text{max}}$ respectively.

We use the two previous steps to show that the cumulative difference in service and rent costs under RR and OPT-OFF in a frame is upper bounded by $2M+\kappa+c_{\text{max}}-c_{\text{min}}$. 
Since the fetch cost under RR and OPT-OFF in a frame is equal, we have that the total cost incurred by RR and OPT-OFF in a frame differs by at most $2M+\kappa+c_{\text{max}}-c_{\text{min}}$. 

We show that once fetched, OPT-OFF hosts  the service for at least $\frac{M}{\kappa-c_{\text{min}}}$ time-slots (Lemma \ref{lem:OPT_slots}). We thus conclude that the total cost incurred by OPT-OFF in a frame is lower bounded by $M + \frac{Mc_{\text{min}}}{\kappa-c_{\text{min}}} $. We use this to upper bound the ratio of the cost incurred by RR and cost incurred by OPT-OFF in the frame.

The cost incurred by RR and OPT-OFF in Frame 0 is equal. We then focus on the last frame. If OPT-OFF does evict the service in the last frame, the analysis is identical to that of the previous frame. Else, we upper bound the ratio of the cost incurred by RR and cost incurred by OPT-OFF in the frame.

The final result then follows from stitching together the results obtained for individual frames. 


\subsection{Proof Outline for Theorem \ref{thm:any_online}}

We divide the class of deterministic online policies into two sub-classes. Any policy in the first sub-class hosts  the service during the first time-slot. All other polices are in the second sub-class. 

For each policy in either sub-class, we construct a specific arrival sequence,   a specific rent cost sequence  and compute the ratio of the cost incurred by the deterministic online policy and an alternative policy. By definition, this ratio serves as a lower bound on the competitive ratio of the deterministic online policy.

\subsection{Proof Outline for Theorem \ref{thm:RR_stochastic_theorem}}

We first characterize a lower bound on the cost per time-slot incurred by any online policy (Lemma \ref{lemma:optimal_causal}).

Next, we focus on the case where $\mu > c$. We upper bound the probability of the service not being hosted during time-slot $t$ under RR  using Hoeffding's inequality \cite{hoeffding1994probability}. The result then follows by the fact that conditioned on the service being hosted in time-slot $t$, the expected total cost incurred by RR  is at most $\mathbb{E}[R_t]+\mathbb{E}[X_t - \min\{X_t, \kappa\}] = c + \mathbb{E}[X_t] - \mu$ and is upper bounded by $M + c + \mathbb{E}[X_t]$ otherwise. 
We then consider the case where $\mu < c$. We upper bound the probability of the service being hosted or being fetched in time-slot $t$ under RR  using Hoeffding's inequality  \cite{hoeffding1994probability}. The result then follows by the fact that conditioned on the service not being hosted and not being fetched in time-slot $t$, the expected total cost incurred by RR is at most $\mathbb{E}[X_t]$ and is upper bounded by $M + c + \mathbb{E}[X_t]$ otherwise. 
\subsection{Proof Outline for Theorem \ref{thm:fixed_TTL}}
Depending on the value of the system parameters ($M$, $c_{\text{min}}$, $c_{\text{max}}$, $\kappa$), we construct specific arrival sequences,  rent cost sequences and compute the ratio of the cost incurred by TTL and OPT-OFF for these  sequences. By definition, this ratio serves as a lower bound on the competitive ratio of TTL in each case.
\subsection{Proof Outline for Theorem \ref{thm:TTL_stochastic_theorem}}
Under the TTL policy with TTL value $L$, the service is hosted during a given time-slot if and only if it is requested at least once in the $L$ previous time-slots. We compute the probability of the event $G$ defined as the event that the service is requested at least once in the $L$ previous time-slots. We compute the conditional expected cost incurred by the TTL policy in time-slot conditioned on $G$ and $G^c$ to obtain the result.

==> proofs.tex <==
\subsection{Proof of Theorem \ref{thm:RR_adv}}
The notation used in this subsection is given in Table \ref{table:proofs}. 
\begin{table}[ht]
	\centering
	\begin{tabular}{ |c | l|} 
		\hline
		\textbf{Symbol}&  \textbf{Description} \\ 
		\hline
		\hline
		$t$ & Time index\\
		\hline
		$M$ & Fetch cost\\
		\hline
		$c_t$       & Rent cost per time-slot  $t$\\
		\hline
		$c_{\text{min}}$       &Minimum value of $c_t$\\
		\hline
		$c_{\text{max}}$       &Maximum value of $c_t$\\
		\hline
		
		$x_t$       & Number of requests arriving in time-slot $t$\\
		\hline
		$\underbar{\text{$x$}}_t$       & $\min \{x_t, \kappa\}$ \\
		\hline
		$\delta_t$       & $x_t-\underbar{\text{$x$}}_t$\\
		\hline
		$r^*(t)$   & Indicator variable; 1 if the service is hosted  by OPT-OFF during time-slot $t$ and 0 otherwise \\
		\hline
		$\text{  }$  &  $\text{ }$\\
		$r^{\text{RR}}(t)$   & Indicator variable; 1 if the service is hosted  by RR during time-slot $t$ and 0 otherwise \\
		\hline
		$\eta$   & a policy\\
		\hline
		$\text{  }$  &  $\text{ }$\\
		$C^{\eta}(n,m)$   & Total cost incurred by the policy $\eta$ in the	 interval $[n,m]$\\
		\hline
		$\text{  }$  &  $\text{ }$\\
		$C^{\text{OPT-OFF}}(n,m)$  & Total cost incurred by the offline optimal policy in the interval $[n,m]$\\
		\hline
		Frame $i$  & The interval between the $i^{\text{th}}$ and the $(i+1)^{\text{th}}$ fetch by the offline optimal policy\\
		\hline
		$\text{  }$  &  $\text{ }$\\
		$C^{\text{OPT-OFF}}(i)$   & Total cost incurred by the offline optimal policy in Frame $i$\\
		\hline
		$\text{  }$  &  $\text{ }$\\
		$C^{\text{RR}}(i)$   & Total cost incurred by RR in Frame $i$\\
		\hline
	\end{tabular}
	\vspace*{10pt}
	\caption{Notation}
	\vspace*{-10pt}
	\label{table:proofs}
\end{table}

We use the following lemmas to prove Theorem \ref{thm:RR_adv}. 

The first lemma gives a lower bound on the number of requests that can be served by the edge server in the time-interval starting from a fetch to the subsequent eviction by OPT-OFF.
\begin{lemma}\label{lem:lemma_opt}
	
	If $r^*(n-1) = 0$, $r^*(t) = 1$ for $n \leq t \leq m$ and $r^*(m+1) = 0$, then,  
	$
	\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l \geq M+	\displaystyle\sum_{l=n}^m c_l.
	$
\end{lemma}
\begin{proof}
	The cost incurred by OPT-OFF in $n \leq t \leq m$ is $M+\displaystyle\sum_{l=n}^m c_l+\displaystyle\sum_{l=n}^m \delta_l.$ We prove Lemma \ref{lem:lemma_opt} by contradiction. Let us assume that $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l < M+\displaystyle\sum_{l=n}^m c_l$. We construct another policy $\eta$ which behaves same as OPT-OFF except that $r_{\eta}(t) = 0$ for $n \leq t \leq m$.
	The total cost incurred by $\eta$ in $n \leq t \leq m$ is $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l+\displaystyle\sum_{l=n}^m\delta_l.$ It follows that
	$C^{\eta}(n,m)-C^{\text{OPT-OFF}}(n,m)= \displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l-M-\displaystyle\sum_{l=n}^m c_l,$ which is negative by our assumption. This contradicts the definition of the OPT-OFF policy, thus proving the result.
\end{proof}
The next lemma shows that if the number of requests that can be served by the edge server in a time-interval exceeds a certain value (which is a function of the length of that time-interval) and the service is not hosted  at the beginning of this time-interval, then OPT-OFF fetches the service at least once in the time-interval. 
\begin{lemma}\label{lem:OPT_download}
	If $r^*(n-1) = 0$, and $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l \geq M+\displaystyle\sum_{l=n}^m c_l$, then OPT-OFF fetches the service at least once in the interval from time-slots $n$ to $m$.
\end{lemma}
\begin{proof}
	We prove Lemma \ref{lem:OPT_download} by contradiction. We  construct another policy $\eta$ which behaves same as OPT-OFF except that $r_{\eta}(t) = 1$ for $n \leq t \leq m$. 
	The total cost incurred by $\eta$ in $n \leq t \leq m$ is $C^{\eta}(n,m)=M+\displaystyle\sum_{l=n}^m c_l+\displaystyle\sum_{l=n}^m \delta_l$. It follows that
	$C^{\eta}(n,m)-C^{\text{OPT-OFF}}(n,m)= M+\displaystyle\sum_{l=n}^m c_l-\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l,$ which is negative. Hence there exists at least one policy $\eta$ which performs better than OPT-OFF. This contradicts the definition of the OPT-OFF policy, thus proving the result.
\end{proof}

The next lemma provides a lower bound on the duration for which OPT-OFF hosts  the service once it is fetched.
\begin{lemma}\label{lem:OPT_slots}
	Once OPT-OFF fetches the service, it is hosted  for at least $\frac{M}{\kappa-c_{\text{min}}}$ slots.
\end{lemma}
\begin{proof}
	Suppose OPT-OFF fetches the service at the end of the $(n-1)^{\text{th}}$ time-slot and evicts it at the end of time-slot $m > n$. From Lemma \ref{lem:lemma_opt}, $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l \geq M+\displaystyle\sum_{l=n}^m c_l$. Since $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l\leq (m-n+1)\kappa$ and $\displaystyle\sum_{l=n}^m c_l\geq (m-n+1)c_{\text{min}}$, $(m-n+1)\kappa \geq M+(m-n+1)c_{\text{min}}$, i.e, $(m-n+1) \geq \frac{M}{\kappa-c_{\text{min}}}$. This proves the result.
\end{proof}


Our next lemma characterizes a necessary condition for RR to fetch the service. 
\begin{lemma}\label{lem:RR_slots}
	If $r^{\text{RR}}(n) = 0$ and $r^{\text{RR}}(n+1) = 1$, then, by the definition of the RR policy, $\exists \tau < n$ such that $\displaystyle\sum_{l=n-\tau+1}^n \underbar{\text{$x$}}_l\geq \displaystyle\sum_{l=n-\tau+1}^n c_l +M.$
	Let $\tau_{\text{min}}=\displaystyle\min_\tau \left\{\tau|\displaystyle\sum_{l=n-\tau+1}^n \underbar{\text{$x$}}_l \geq \displaystyle\sum_{l=n-\tau+1}^n c_l +M\right\}$. Then,  
	$\tau_{\text{min}} \geq \frac{M}{\kappa-c_{\text{min}}}.$
\end{lemma}
\begin{proof}
	Since $\displaystyle\sum_{l=n-\tau+1}^n \underbar{\text{$x$}}_l	\leq \tau \kappa$, $\tau_{\text{min}} \kappa \geq \tau_{\text{min}} c_{\text{min}}+M$, and the result follows. 
\end{proof}



The next lemma gives an upper bound on the number of requests that can be served by the edge server (subject to its computation power constraints) in a time-interval such that RR does not host  the service during the time-interval and fetches it in the last time-slot of the time-interval. 


\begin{lemma}\label{lem:max_requests}
	Let $r^{\text{RR}}(n-1)=1$, $r^{\text{RR}}(t)=0$ for $n \leq t \leq m$ and $r^{\text{RR}}(m+1)=1$. Then for any $n\leq n'< m$,  $\displaystyle\sum_{l=n'}^m \underbar{\text{$x$}}_l < \displaystyle\sum_{l=n'}^{m-1} c_l+M+\kappa.$   
\end{lemma}
\begin{proof}
	Given $r^{\text{RR}}(m)=0$ and $r^{\text{RR}}(m+1)=1$, then for any $n\leq n'< m$, $\displaystyle\sum_{l=n'}^{m-1} \underbar{\text{$x$}}_l <  \displaystyle\sum_{l=n'}^{m-1} c_l+M.$ 
	By definition,
	$
	\displaystyle\sum_{l=n'}^m \underbar{\text{$x$}}_l= \left(\displaystyle\sum_{l=n'}^{m-1} \underbar{\text{$x$}}_l\right)+\underbar{\text{$x$}}_{m}< \displaystyle\sum_{l=n'}^{m-1} c_l+M+\kappa,
	$
	thus proving the result.	
\end{proof}



Consider the event where both RR and OPT-OFF have hosted  the service in a particular time-slot. The next lemma states that given this, OPT-OFF evicts the service before RR. 

\begin{lemma}\label{lem:eviction}
	If $r^{\text{RR}}(n)=1$, $r^*(t) = 1$ for $n \leq t \leq m$, and $r^*(m+1) = 0$. Then,  $r^{\text{RR}}(t)=1$ for $n+1 \leq t \leq m+1$.
\end{lemma}
\begin{proof}
	We prove this by contradiction. Let $\exists \widetilde{m}<m$ such that $r^{\text{RR}}(\widetilde{m}+1)=0$. Then, from Algorithm \ref{algo:RR}, there exists an integer $\tau>0$  such that  $\displaystyle\sum_{l=\widetilde{m}-\tau+1}^{\widetilde{m}} \underbar{\text{$x$}}_l< \displaystyle\sum_{l=\widetilde{m}-\tau+1}^{\widetilde{m}} c_l-M.$ 	The cost incurred by OPT-OFF in the interval $\widetilde{m}-\tau+1$ to $\widetilde{m}$ is $\displaystyle\sum_{l=\widetilde{m}-\tau+1}^{\widetilde{m}} c_l+\displaystyle\sum_{l=\widetilde{m}-\tau+1}^{\widetilde{m}}\delta_l$. 
	
	Consider an alternative policy $\eta$ for which $r_{\eta}(t)=0$ for $\widetilde{m}-\tau+1 \leq t \leq \widetilde{m}$, $r_{\eta}(\widetilde{m}+1)=1$, and $r_{\eta}(t)=r^*(t)$ otherwise. It follows that
	$C^{\eta}-C^{\text{OPT-OFF}}= \displaystyle\sum_{l=\widetilde{m}-\tau+1}^{\widetilde{m}} \underbar{\text{$x$}}_l + M  - \displaystyle\sum_{l=\widetilde{m}-\tau+1}^{\widetilde{m}} c_l$ which is negative by our assumption. This contradicts the definition of the OPT-OFF policy, thus proving the result.	
\end{proof}

Consider the case where both RR and OPT-OFF have hosted  the service in a particular time-slot. From the previous lemma, we know that, OPT-OFF evicts the service before RR. The next lemma gives a lower bound on the number of requests that can be served by the edge server (subject to its computation power constraints) in the interval which starts when OPT-OFF evicts the service from the edge server  and ends when RR evicts the service from the edge server. 
\begin{lemma}\label{lem:min_requests}
	Let $r^*(n-1)= 1, \ r^*(n)=0, \ r^{\text{RR}}(t) = 1$ for $n-1 \leq t \leq m$ and  $r^{\text{RR}}(m+1)=0$.Then for any $n\leq n'< m$, $\displaystyle\sum_{l=n'}^m \underbar{\text{$x$}}_l \geq 	\displaystyle\sum_{l=n'}^{m-1} c_l-M.$    	
\end{lemma}
\begin{proof}
	Given $r^{\text{RR}}(m)=1$ and $r^{\text{RR}}(m+1)=0$, then  for any $n\leq n'< m$, $\displaystyle\sum_{l=n'}^{m-1} \underbar{\text{$x$}}_l > 	\displaystyle\sum_{l=n'}^{m-1} c_l-M$. 
	%we have that $\exists \tau >0$   such that $\displaystyle\sum_{l=m-\tau+1}^m \underbar{\text{$x$}}_l < \tau c-M$ and $\displaystyle\sum_{l=n}^{m-1} \underbar{\text{$x$}}_l \geq (m-n) c-M$. 
	By definition,
	$
	\displaystyle\sum_{l=n'}^m \underbar{\text{$x$}}_l= \left(\displaystyle\sum_{l=n'}^{m-1} \underbar{\text{$x$}}_l\right)+\underbar{\text{$x$}}_{m}> \displaystyle\sum_{l=n'}^{m-1} c_l-M+0,
	$
	thus proving the result. 	
\end{proof}
Our next result states that RR does not fetch the service in the interval between an eviction and the subsequent fetch by OPT-OFF.

\begin{lemma}\label{lem:RR_no_download} If $r^*(n-1) = 1, \ r^*(t) = 0$ for $n \leq t \leq m$, and $r^*(m+1)=1$, then RR does not fetch the service in time-slots $n, n+1, \cdots, m-1$. 
\end{lemma}

\begin{proof}
	We prove this by contradiction. Let RR fetch the service in time-slot $t$ where $n\leq t \leq m-1.$ 
	Then from Algorithm \ref{algo:RR}, there exists an integer $\tau>0$ such that $t-\tau\geq n$ and $\displaystyle\sum_{l=t-\tau+1}^t \underbar{\text{$x$}}_l\geq \displaystyle\sum_{l=t-\tau+1}^t c_l+M.$
	If this condition is true, by Lemma \ref{lem:OPT_download},  OPT-OFF would have fetched the service at least once in the interval $t-\tau+1$ and $t$ for all $n\leq t \leq m-1.$ Hence RR does not fetch the service between $n$ and $m-1.$
\end{proof}






The next lemma states that in the interval between a fetch and the subsequent eviction by OPT-OFF, RR hosts  the service for at least one time-slot. 

\begin{lemma}\label{lem:RR_one_download}
	If $r^*(n-1) = 0$, $r^*(t) = 1$ for $n \leq t \leq m$ and $r^*(m+1) = 0$, then,
	for some  $n < t \leq m$, $r^{\text{RR}}(t) = 1.$
\end{lemma}
\begin{proof}
	We prove this by contradiction. Let $r^{\text{RR}}(t)=0$ for all $n \leq t \leq m$. Then by the definition of the RR policy,  $\displaystyle\sum_{l=t-\tau+1}^t \underbar{\text{$x$}}_l < \displaystyle\sum_{l=t-\tau+1}^t c_l+M$ for any $\tau>0$ and $\tau \leq t-n+1$.
	If we choose $t=m$   then  $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l < \displaystyle\sum_{l=n}^m c_l+M$, which is false from Lemma \ref{lem:lemma_opt}. This contradicts our assumption.  
\end{proof}



If both RR and OPT-OFF host  the service in a particular time-slot, from Lemma \ref{lem:eviction}, we know that OPT-OFF evicts the service before RR. The next lemma states that RR evicts the service before the next time OPT-OFF fetches it. 
\begin{lemma}\label{lem:RR_one_evict}
	If $r^*(n-1) = 1$, $r^*(t) = 0$ for $n \leq t \leq m$, $r^*(m+1) = 1$, and $r^{\text{RR}}(n-1)=1$, then, RR evicts the service by the end of time-slot $m$ and $r^{\text{RR}}(m+1) = 0$.
\end{lemma}
\begin{proof}
	We prove this by contradiction. Assume that RR does not evict the service in any time slot $t$ for all  $n \leq t \leq m$. 
	Then from the definition of the RR policy, $\displaystyle\sum_{l=t-\tau+1}^{t} \underbar{\text{$x$}}_l+M \geq \displaystyle\sum_{l=t-\tau+1}^{t} c_l$ for all $\tau$ such that $0 < \tau \leq t-n+1$.
	As a result, at $t=m$, $\displaystyle\sum_{l=n}^m \underbar{\text{$x$}}_l +M > \displaystyle\sum_{l=n}^m c_l$. 
		Given this, it follows that OPT-OFF will not evict the service at the end of time-slot $n-1$. 
	This contradicts our assumption.
	By Lemma \ref{lem:RR_no_download}, RR does not fetch the service in the interval between an eviction and the subsequent fetch by OPT-OFF. Therefore, $r^{\text{RR}}(m+1) = 0$.
\end{proof}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 


To compare the costs incurred by RR and OPT-OFF we divide time into frames $[1,t_1-1]$, $[t_1,t_2-1], [t_2,t_3-1],\cdots,$ where $t_i-1$ is the time-slot in which OPT-OFF fetches the service for the $i^{\text{th}}$ time for $i\in\{1,2,\cdots\}.$ Our next result characterizes the sequence of events that occur in any such frame.



\begin{lemma}
	\label{lem:frameStructure}
	Consider the interval $[t_i, t_{i+1}-1]$ such that OPT-OFF fetches the service at the end of time-slot $t_{i}-1$ and fetches it again the end of time-slot $t_{i+1}-1$. By definition, there exists $\tau \in [t_i, t_{i+1}-2]$ such that OPT-OFF evicts the service in time-slot $\tau$. 
	RR fetches and evicts the service exactly once each in $[t_1, t_2-1]$. The fetch by RR is in time-slot $t_{f}^{\text{RR}} $ such that $t_1 \leq t_{f}^{\text{RR}} \leq \tau$ and
	the eviction by RR is in time-slot $t_{e}^{\text{RR}}$ such that $\tau < t_{e}^{\text{RR}} < t_2$ (Figure \ref{fig:OPT_RR_frame}).
\end{lemma}


\begin{figure}[ht]
	\centering
	\begin{tikzpicture}
	\foreach \x in {0,0.3,0.6,...,7.2}{
		\draw[] (\x,0) --  (\x+0.3,0);
		\draw[gray] (\x,-1mm) -- (\x,1mm);
	}
	
	\draw[gray] (7.2,-1mm) -- (7.2,1mm);
	\draw[-latex] (0.25,10mm) -- node[above=5mm]{$t_{i}-1$} (0.25,0mm);
	\draw[-latex] (6.85,10mm) -- node[above=5mm]{$t_{i+1}-1$} (6.85,0mm);
	\draw[-latex] (4.15,0mm) -- node[above=5mm]{$\tau$} (4.15,10mm);
	\draw[-latex,color=red] (2.35,10mm) -- node[above=5mm]{$t_f^{\text{RR}}$} (2.35,0mm);
	\draw[-latex,color=red] (5.65,0mm) -- node[above=5mm]{$t_e^{\text{RR}}$} (5.65,10mm);
	
	\draw[gray] (7.2,-1mm) -- (7.2,1mm);
	\draw[-latex] (0.25,10mm) -- node[above=5mm]{} (0.25,0mm);
	\draw[-latex] (6.85,10mm) -- node[above=5mm]{} (6.85,0mm);
	\draw[-latex] (4.15,0mm) -- node[above=5mm]{} (4.15,10mm);
	\draw[-latex,color=red] (2.35,10mm) -- node[above=5mm]{} (2.35,0mm);
	\draw[-latex,color=red] (5.65,0mm) -- node[above=5mm]{} (5.65,10mm);
	
	\draw[<->,color=black] (0.3,-2mm) -- node[below=0mm,pos=0.5]{Frame $i$} (6.9,-2mm);
	
	\draw[black] (0.3,-1mm) -- (0.3,-3mm);
	\draw[black] (6.9,-1mm) -- (6.9,-3mm);
	
	\node[] at (7.7,-0.9) {OPT-OFF};
	
	\filldraw[fill=black!] (0.25,-1) rectangle (4.15,-0.7);
	\filldraw[fill=white!40] (4.15,-1) rectangle (6.85,-0.7);
	\node[] at (7.25,-1.4) {RR};
	\filldraw[fill=white!40] (0.25,-1.5) rectangle (2.4,-1.2);
	\filldraw[fill=red!] (2.4,-1.5) rectangle (5.7,-1.2);
	\filldraw[fill=white!40] (5.7,-1.5) rectangle (6.85,-1.2);
	
	
	\end{tikzpicture}
	\caption{Illustration of Lemma \ref{lem:frameStructure} showing download and eviction by OPT-OFF and  RR in the $i^{\text{th}}$ frame. Downward arrows represent fetches, upward arrows indicate evictions. Black and red arrows correspond to the OPT-OFF and RR policy respectively. The two bars below the timeline indicate the state of the edge server  under OPT-OFF and RR. The solid black and solid red portions represent the intervals during with OPT-OFF and RR host  the service on the edge server respectively}
	\label{fig:OPT_RR_frame}
	%\vspace*{-10pts}
\end{figure}


\begin{proof}
	Without loss of generality, we prove the result for $i=1$.
	Since $r^*(t_1-1) = 0$, $r^*(t) = 1$ for $t_1 \leq t \leq \tau$ and $r^*( \tau) = 0$ then by Lemma \ref{lem:RR_one_download}, $r^{\text{RR}}(t_{f}^{\text{RR}}) = 1$ for some  $t_1 < t_{f}^{\text{RR}} \leq \tau.$ In addition, by Lemma \ref{lem:RR_one_evict}, $r^{\text{RR}}(t_1) = 0$. Therefore, RR fetches the service at least once in the interval $[t_1, t_2-1]$.%, such that the fetch by RR is in time-slot $t_{f}^{\text{RR}} $, $t_1 \leq t_{f}^{\text{RR}} \leq \tau$. 
		By Lemma \ref{lem:eviction}, if $t_{f}^{\text{RR}} < \tau$, since both RR and OPT-OFF host  the service during time-slot $t_{f}^{\text{RR}}+1$, OPT-OFF evicts the service before RR, therefore, once fetched, RR does not evict the service before time-slot $\tau+1$, i.e., $r^{\text{RR}}(t)=1$ for $t_{f}^{\text{RR}}+1 \leq t \leq \tau+1.$
		Since $r^*(\tau) = 1$, $r^*(t) = 0$ for $\tau+1 \leq t \leq t_2-1$ and $r^*(t_2) = 1$, then by Lemma \ref{lem:RR_one_evict}, RR evicts the service in time-slot $t_{e}^{\text{RR}}$ such that $\tau < t_{e}^{\text{RR}} \leq t_2-1$.
	In addition, once evicted at $t_{e}^{\text{RR}} \leq t_2-1$, RR does not fetch it again in the before time-slot $t_2$ by Lemma \ref{lem:RR_no_download}. 
		This completes the proof.
\end{proof}



\begin{proof}[Proof of Theorem \ref{thm:RR_adv} ] As mentioned above, to compare the costs incurred by RR and OPT-OFF we divide times into frames $[1,t_1-1]$, $[t_1,t_2-1], [t_2,t_3-1],\ldots,$ where $t_i-1$ is the time-slot in which OPT-OFF downloads the service for the $i^{\text{th}}$ time for $i\in\{1,2,\ldots, k\}.$ 
	
	
	
	For convenience, we account for the fetch cost incurred by OPT-OFF in time-slot $t_i$ in the cost incurred by OPT-OFF in Frame $i$. Given this, the cost under RR and OPT-OFF is the same for $[1,t_1-1]$ (Frame 0) since both policies don't host  the service in this period. 
	
	Note that if the total number of fetches made by OPT-OFF is $k<\infty$, there are exactly $k+1$ frames (including Frame 0). The $(k+1)^{\text{th}}$ frame either has no eviction by OPT-OFF or OPT-OFF evicts and then never fetches the service. 
	
	We now focus on Frame $i$, such that $0<i<k$, where $k$ is the total number of fetches made by OPT-OFF. 
	
	
	
	Without loss of generality, we focus on Frame 1. Recall the definitions of $\tau$, $t_e^{\text{RR}}$, and $t_f^{\text{RR}}$ from Lemma \ref{lem:frameStructure}, also seen in Figure \ref{fig:OPT_RR_frame}. By Lemma \ref{lem:frameStructure}, we have that RR fetches and evicts the service exactly once each in $[t_1, t_2-1]$ such that the fetch by RR is in time-slot $t_{f}^{\text{RR}} $ such that $t_1 \leq t_{f}^{\text{RR}} \leq \tau$ and 
	the eviction by RR is in time-slot $t_{e}^{\text{RR}}$ such that $\tau < t_{e}^{\text{RR}} < t_2$.
	
	Both OPT-OFF and RR makes one fetch in the frame. Hence the difference in the fetch costs is zero. We now focus on the service and rent cost incurred by the two policies. 
	%\begin{itemize}
	%\item [--]  
	
	By Lemma \ref{lem:max_requests}, the number of requests that can be served by the edge server in $[t_1, t_{f}^{\text{RR}}]$ is at most $M+\displaystyle \sum_{l = t_1}^{t_{f}^{\text{RR}}} c_l +\kappa.$ 
	Since RR does not host  the service in $[t_1, t_{f}^{\text{RR}}]$, the rent cost incurred in $[t_1, t_{f}^{\text{RR}}]$ by RR is zero and the service cost incurred in $[t_1, t_{f}^{\text{RR}}]$ by RR 
	is at most $M+\displaystyle \sum_{l = t_1}^{t_{f}^{\text{RR}}-1} c_l +\kappa + \displaystyle \sum_{l = t_1}^{t_{f}^{\text{RR}}} \delta_l$. OPT-OFF rents storage in $[t_1, t_{f}^{\text{RR}}]$ at cost $ \displaystyle \sum_{l = t_1}^{t_{f}^{\text{RR}}} c_l$ and incurs a service cost of $\displaystyle \sum_{l = t_1}^{t_{f}^{\text{RR}}} \delta_l$ in $[t_1, t_{f}^{\text{RR}}]$. 
	Hence difference in the service and rent cost incurred by RR and OPT-OFF in $[t_1, t_{f}^{\text{RR}}]$   is at most $M+\kappa-c_{\text{min}}.$
	%\item[--] 
		The service and rent cost incurred by OPT-OFF and RR in $[t_{f}^{\text{RR}}+1, \tau]$ are equal. 
	%\item [--] 
	By Lemma \ref{lem:min_requests}, the number of requests that can be served by the edge server in $[\tau+1, t_{e}^{\text{RR}}]$ is at least $ \displaystyle \sum_{l = \tau+1}^{t_{e}^{\text{RR}}-1} c_l-M.$ The service cost incurred by OPT-OFF in $[\tau+1, t_{e}^{\text{RR}}]$ is at least $\displaystyle \sum_{l = \tau+1}^{t_{e}^{\text{RR}}-1} c_l-M + \displaystyle \sum_{l = \tau+1}^{t_{e}^{\text{RR}}} \delta_l$ and the rent cost incurred by OPT-OFF in $[\tau+1, t_{e}^{\text{RR}}]$ is zero. The rent cost incurred by RR in $[\tau+1, t_{e}^{\text{RR}}]$ is $\displaystyle \sum_{l = \tau+1}^{t_{e}^{\text{RR}}} c_l$ and the service cost incurred by RR in $[\tau+1, t_{e}^{\text{RR}}]$ is $\displaystyle \sum_{l = \tau+1}^{t_{e}^{\text{RR}}} \delta_l$. Hence difference in the service and rent cost incurred by RR and OPT-OFF in $[t_1, t_{f}^{\text{RR}}]$  is at most $M+c_{\text{max}}.$
	
	% \item[--] 
	The service and rent cost incurred by OPT-OFF and RR in $[t_{e}^{\text{RR}}+1, t_2-1]$ are equal. 
	%\end{itemize}
	
	Let $C^{\text{RR}}(i),$ $C^{\text{OPT-OFF}}(i)$ denote the costs incurred in the $i^{\text{th}}$ frame by RR and OPT-OFF respectively.
	We therefore have that,
	$
	C^{\text{RR}}(i)-C^{\text{OPT-OFF}}(i)\leq 2M+\kappa+c_{\text{max}}-c_{\text{min}}.
	$

	Since $c_{\text{max}}\leq M+\kappa$, we have that,
	\begin{align}
	C^{\text{RR}}(i)-C^{\text{OPT-OFF}}(i)&\leq 3M+2\kappa.
	\label{ineq:bound1_RR}
	\end{align}
	
	By Lemma \ref{lem:OPT_slots}, once OPT-OFF downloads the service, it is hosted  for at least $\frac{M}{\kappa-c_{\text{min}}}$ slots. Therefore,
	\begin{align}
	&C^{\text{OPT-OFF}}(i)\geq M+\frac{Mc_{\text{min}}}{\kappa-c_{\text{min}}} \implies C^{\text{OPT-OFF}}(i)\geq \frac{M\kappa}{\kappa-c_{\text{min}}}\nonumber\\
	&M\leq \frac{\kappa-c_{\text{min}}}{\kappa}C^{\text{OPT-OFF}}(i) \text{ and } \kappa\leq \frac{\kappa-c_{\text{min}}}{M}C^{\text{OPT-OFF}}(i).
	\label{ineq:bound1_OPT}
	\end{align}
	
	From \eqref{ineq:bound1_RR} and \eqref{ineq:bound1_OPT}, 
	\begin{align}
	C^{\text{RR}}(i) \leq \left(4-\frac{3c_{\text{min}}}{\kappa}\right)C^{\text{OPT-OFF}}(i)+2\left(\frac{\kappa-c_{\text{min}}}{M}\right)C^{\text{OPT-OFF}}(i)
	 \leq \left(4+\frac{2(\kappa-c_{\text{min}})}{M}-\frac{3c_{\text{min}}}{\kappa}\right)C^{\text{OPT-OFF}}(i).
	\end{align}
	
	
	This completes the characterization for Frame $1$ to $k-1$.
	
	We now focus on Frame $k$, which is the last frame. There are two possible cases, one where OPT-OFF evicts the service in Frame $k$, in which case the analysis for Frame $k$ is identical to that of Frame $1$, and the other when OPT-OFF does not evict the service in Frame $k$. We now focus on the latter. 
	
	%
	
	Given that OPT-OFF downloads the service in time-slot $t_{k}-1$, there exists $m>t_{k}$ such that
	$\displaystyle\sum_{l=t_k}^m \underbar{\text{$x$}}_l \geq M+\displaystyle\sum_{l=t_k}^m c_l$.
	By Step~8 in Algorithm \ref{algo:RR}, RR downloads the service at the end of
	time-slot $m$.
	Let $\tau_k = m-t_k$. By Lemma \ref{lem:max_requests}, the number of requests that can be served by the edge server during these $\tau_k$ time-slots is at most $M+\displaystyle\sum_{l=t_k}^{m-1} c_l+\kappa.$
	Since RR does not host  the service during these  $\tau_k$ time-slots, the rent cost incurred by RR is zero and the service cost incurred by RR is at most $M+\displaystyle\sum_{l=t_k}^{m-1} c_l+\kappa + \displaystyle \sum_{l = t_k}^{m} \delta_l$. OPT-OFF rents storage during these $\tau_k$ time-slots at cost $\displaystyle \sum_{l = t_k}^{m} c_l$ and the service cost incurred by OPT-OFF is $\displaystyle \sum_{l = t_k}^{m - 1} \delta_l$. There is no difference between the cost of RR and OPT-OFF after the first $\tau_k$ slots in Frame $k$. It follows that
	\begin{align}
	C^{\text{RR}}(k)-C^{\text{OPT-OFF}}(k)\leq M+\kappa-c_{\text{min}}.
	\label{ineq:bound1_RRk}
	\end{align}
	%By Lemma \ref{lem:OPT_slots}, once OPT downloads the service, it is host s for at least $\frac{M}{\kappa-c}$ slots. Therefore,
	%\begin{align}
	%C_{\text{OPT}}(k)\geq M+\frac{Mc}{\kappa-c} \implies M\leq \frac{\kappa-c}{\kappa}C_{\text{OPT}}(k).
	%\label{ineq:bound1_OPTk}
	%\end{align}
	From \eqref{ineq:bound1_OPT} and \eqref{ineq:bound1_RRk},

	\begin{align}
	C^{\text{RR}}(k) &\leq \left(2-\frac{c_{\text{min}}}{\kappa}\right)C^{\text{OPT-OFF}}(k)+\left(\frac{\kappa-c_{\text{min}}}{M}\right)C^{\text{OPT-OFF}}(k)
	 < \left(4+\frac{2(\kappa-c_{\text{min}})}{M}-\frac{3c_{\text{min}}}{\kappa}\right)C^{\text{OPT-OFF}}(k).
	\end{align}

	
	Stitching together the results obtained for all frames, the result follows.  
	
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:any_online}}
\begin{proof}
	Let $\mathcal{P}$ be a given deterministic online policy and $C^\mathcal{P}(a,b)$ be the cost incurred by this policy for the request sequence $a$ and rent cost sequence $b$.
	
	We first focus on the case where $\mathcal{P}$ does not host  the service during the first time-slot. 
	
	We define $t_\text{fetch}^{(1)}\geq1$ as the first time the policy $\mathcal{P}$ fetches the service when there are $\kappa$ request arrivals each in the first $t_\text{fetch}^{(1)}$ time-slots. Since $\mathcal{P}$ is an online deterministic policy, the value of $t_\text{fetch}^{(1)}$ can be computed a-priori.
	
	Consider the arrival process $a$ with $\kappa$ request arrivals each in the first $t_\text{fetch}^{(1)}$ time-slots and no arrivals thereafter.
	Consider a renting cost sequence $b$ with  $c_{\text{min}}$ in the first $t_\text{fetch}^{(1)}$ time-slots.
	It follows that $C^{\mathcal{P}}(a,b) \geq \kappa t_\text{fetch}^{(1)} + M + c_{\text{min}}.$
	
	Consider an alternative policy ALT which hosts  the service in time-slots $1$ to $t_\text{fetch}^{(1)}$ and does not host  it thereafter. It follows that $C^{\text{ALT}}(a,b) = c_{\text{min}} t_\text{fetch}^{(1)} + M.$
	By definition,
	$
	\rho^{\mathcal{P}} \geq \dfrac{\kappa t_\text{fetch}^{(1)} + M + c_{\text{min}}}{c_{\text{min}} t_\text{fetch}^{(1)} + M}. %&\geq 1 + \dfrac{(\kappa - c) t_\text{fetch}^{(1)} + c}{c t_\text{fetch}^{(1)} + M}.
	$
	Therefore,
	\begin{align*}
	\rho^{\mathcal{P}} \geq
	\begin{cases*}
	1 + \dfrac{\kappa}{c_{\text{min}} + M} \hspace{1em} \text{ if } \kappa \geq \dfrac{c_{\text{min}}(c_{\text{min}}+M)}{M} \\
	\dfrac{\kappa}{c_{\text{min}}} \hspace{4.8em} \text{ otherwise. }
	\end{cases*}
	\end{align*}
	
	Next, we focus on the case where $\mathcal{P}$ hosts  the service during the first time-slot. We define $t_\text{evict}^{(1)}\geq1$ as the first time the policy $\mathcal{P}$ evicts the service when there are no request arrivals each in the first $t_\text{evict}^{(1)}$ time-slots. Since $\mathcal{P}$ is an online deterministic policy, the value of $t_\text{evict}^{(1)}$ can be computed a-priori.
	
	Consider the arrival process $a$ with no request arrivals each in the first $t_\text{evict}^{(1)}$ time-slots and $\kappa$ arrivals in time-slot $t_\text{evict}^{(1)}+1$.
	Consider the renting cost sequence $b$ with $c_{\text{max}}$ each in the first $t_\text{evict}^{(1)}$ time-slots and $c_{\text{min}}$  in time-slot $t_\text{evict}^{(1)}+1$.
	It follows that $C^{\mathcal{P}}(a,b) \geq c_{\text{max}} t_\text{evict}^{(1)} + M + \kappa.$ Consider an alternative policy ALT which does not host  the service in time-slots $1$ to $t_\text{evict}^{(1)}$, hosts  it in time-slot $t_\text{evict}^{(1)}+1$ and does not host  it thereafter. It follows that $C^{\text{ALT}}(a,b) = M + c_{\text{min}}.$
	By definition,
	$
	\rho^{\mathcal{P}} \geq \dfrac{c_{\text{max}} t_\text{evict}^{(1)} + M + \kappa}{M+c_{\text{min}}} %&\geq 1 + \dfrac{(\kappa - c) + c t_\text{evict}^{(1)}}{M +c } \\
	\geq 1 + \dfrac{\kappa+c_{\text{max}}-c_{\text{min}}}{c_{\text{min}}+M}.
$
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem \ref{thm:RR_stochastic_theorem}}
We use the following lemmas to prove Theorem \ref{thm:RR_stochastic_theorem}. 

\begin{lemma}
	\label{lemma:optimal_causal}
	Let $X_t$ be the number  of requests arriving in time-slot $t$, $\nu = \mathbb{E}[X_t]$,  $\underbar{$X$}_t=\min\{X_t,\kappa\}$ and $\mu =  \mathbb{E}[\underbar{$X$}_t]$. 
	Let $R_t$ be the rent cost per time-slot, $\{R_t\}_{t\geq 1}$ is the sequence of negatively associated random variables and $c= \mathbb{E}[R_t]$.
	Under Assumption \ref{assum_stochastic}, let $\mathbb{E}[ C_t^{\text{OPT-ON}}]$ be the cost per time-slot incurred by the OPT-ON policy. Then,
	$
	\mathbb{E}[ C_t^{\text{OPT-ON}}] \geq \min\{c + \nu - \mu, \nu\}.
$
\end{lemma}
\begin{proof}
	If the service is hosted  at the edge in time-slot $t$, the expected cost incurred is at least $\mathbb{E}[X_t +R_t- \min\{X(t) , \kappa\}]$ = $c + \nu - \mu$. %as at most $\kappa$ requests can be served by the edge server. %Since $\mu =  \mathbb{E}[\underbar{$X$}_t]$, this cost is equal to $c + \nu - \mu$.
		If the service is not hosted  at the edge server, the expected cost incurred is at least $\nu$. This proves the result.
\end{proof}

\begin{lemma}\label{lem:Hoeffding}
	Let $X_t$ be the number  of requests arriving in time-slot $t$, $\underbar{$X$}_t=\min\{X_t,\kappa\}$ and $\mu =  \mathbb{E}[\underbar{$X$}_t]$. 
	Let $R_t$ be the rent cost per time-slot, $\{R_t\}_{t\geq 1}$ is the sequence of negatively associated random variables and $c= \mathbb{E}[R_t]$. Define $Y_l=\underbar{$X$}_l-R_l$, and  $Y=\sum\limits_{l=t-\tau+1}^t Y_l$ then $Y$ satisfies,
	
	\noindent for $(c-\mu) \tau + M > 0$,
	$
	\mathbb{P}\left(Y \geq M\right)  \leq \exp\left(-2\frac{((c-\mu)\tau+M)^2}{\tau (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right), %\\
	% &\leq \exp\left(-2\frac{(c-\mu)^2\tau}{\kappa^2}\right),
	$
	and for $(\mu-c) \tau + M > 0$,
	$
	\mathbb{P}\left(Y \leq \tau c-M\right)  \leq \exp\left(-2\frac{((\mu-c)\tau+M)^2}{\tau (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right). %\\
	$
\end{lemma}
\begin{proof}   Using i.i.d. condition of $\{X_t\}_{t\geq 1}$  and  negatively associativity of $\{R_t\}_{t\geq 1}$, it follows that for $s>0$, $\mathbb{E}[\exp(sY)]\leq \prod\limits_{l=t-\tau+1}^t \mathbb{E}[\exp(sY_l)]$.  Moreover,	 $Y_l\in [ -c_{\text{max}}, \kappa-c_{\text{min}}]$. Then the result  follows by Hoeffding's inequality  \cite{hoeffding1994probability, wajc2017negative}. 
\end{proof}
\vspace{-1pt}
\begin{proof}[Proof of Lemma \ref{lemma:difference_RRstochastic}] We first consider the case when $\mu>c$. We define the following events

$E_{t_1,t_2}: \displaystyle\sum_{l=t_1}^{t_2} \underbar{$X$}_l \leq \displaystyle\sum_{l=t_1}^{t_2} R_l - M$, $E^{\tau} =\displaystyle\bigcup_{t_1=1}^{\tau} E_{t_1,\tau}$, $E =\displaystyle\bigcup_{\tau=t-\lceil\frac{\lambda M}{\mu-c}\rceil}^{t-1} E^{\tau}$, $F: \displaystyle\sum_{l=t-\lceil\frac{\lambda M}{\mu-c}\rceil}^{t-1} \underbar{$X$}_l \geq \displaystyle\sum_{l=t-\lceil\frac{\lambda M}{\mu-c}\rceil}^{t-1} R_l+M$.  \\
	
	By Lemma \ref{lem:Hoeffding}, it follows that 
	$\mathbb{P}(E_{t_1,t_2})\leq \exp\left(-2\frac{(\mu-c)^2 (t_2-t_1+1)}{(\kappa+c_{\text{max}}-c_{\text{min}})^2}\right),$ 
	and therefore,
	\begin{align}
	\mathbb{P}(E^{\tau})&\leq \displaystyle \sum_{t_1=1}^{\tau-\lceil\frac{M}{c}\rceil+1} \exp\left(-2\frac{(\mu-c)^2 (\tau-t_1+1)}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right) \leq \frac{\exp\left(-2\frac{(\mu-c)^2 \frac{M}{c}}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}{1-\exp\left(-2\frac{(\mu-c)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}. \label{eq:E_tau}
	\end{align}
	Using \eqref{eq:E_tau} and the union bound,
	
	\begin{align}
	\mathbb{P}(E)\leq \bigg\lceil\frac{\lambda M}{\mu-c}\bigg\rceil \frac{\exp\left(-2\frac{(\mu-c)^2 \frac{M}{c}}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}{1-\exp\left(-2\frac{(\mu-c)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}. \label{eq:E}
	\end{align}
	By Lemma \ref{lem:Hoeffding}, 
	\begin{align}
	\mathbb{P}(F^c)&\leq \exp\left(-2\frac{((\mu-c)\lceil\frac{\lambda M}{\mu-c}\rceil-M)^2}{\frac{\lambda M}{\mu-c}  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)  \leq \exp\left(-2\frac{(\lambda-1)^2M(\mu-c)}{\lambda  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right). \label{eq:F}
	\end{align}
	By \eqref{eq:E} and \eqref{eq:F}, 
	\begin{align}
	\mathbb{P}(E^c \cap F)\geq 1 &- \bigg\lceil\frac{\lambda M}{\mu-c}\bigg\rceil \frac{\exp\left(-2\frac{(\mu-c)^2 \frac{M}{c}}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}{1-\exp\left(-2\frac{(\mu-c)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)} - \exp\left(-2\frac{(\lambda-1)^2M(\mu-c)}{\lambda  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right). \label{eq:EcapF}
	\end{align}
	Consider the event $G = E^c \cap F$ and the following three cases. 
	%\begin{itemize}
	%	\item[--] 
	
	Case 1: The service is hosted  at the edge during time-slot $t -\big\lceil\frac{\lambda M}{\mu-c}\big\rceil$: Conditioned on $E^c$, by the properties of the RR  policy, the service is not evicted from the edge server  in time-slots $t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil$ to $t-1$. It follows that in this case, the service is hosted at the edge server  during time-slot $t$.
	%	\item[--] 
	
	Case 2: The service is not hosted  at the edge during time-slot $t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil$ and is fetched in time-slot $\tilde{\tau}$ such that $t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil + 1 \leq \tilde{\tau} \leq t-2$: Conditioned on $E^c$, by the properties of the RR policy, the service is not evicted from the edge server  in time-slots $\tilde{\tau}+1$ to $t-1$. It follows that in this case, the service is hosted at the edge during time-slot $t$.
	%	\item[--] 
	
	Case 3: The service is not hosted  at the edge during time-slot $t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil$ and is not fetched in time-slots $t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil + 1$ to $t-2$: In this case, in time-slot $t-1$, $t_{\text{evict}} \leq t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil$. Conditioned on $F$, by the properties of the RR policy, condition in Step 8 in Algorithm \ref{algo:RR}   is satisfied for $\tau = t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil$.  It follows that in this case, the service is fetched in time-slot $t-1$ and therefore, the service is  hosted at the edge during time-slot $t$.
	%\end{itemize}
	
	We thus conclude that conditioned on $G = E^c \cap F$, the service is hosted  at the edge during time-slot $t$. 
	We now compute the expected cost incurred by the RR policy. By definition,
	$
	\mathbb{E}[C_t^{\text{RR}}] 
	=  \mathbb{E}[C_t^{\text{RR}}|G] \mathbb{P}(G) +\mathbb{E}[C_t^{\text{RR}}|G^c] \times \mathbb{P}(G^c).
	$
	Note that, 
	$
	\mathbb{E}[C_t^{\text{RR}}|G] = c + \nu-\mu, \ \mathbb{E}[C_t^{\text{RR}}|G^c] \leq M + c + \nu.
	$
	Therefore,
	\begin{align}
	\mathbb{E}[C_t^{\text{RR}}] 
	= &  c + \nu-\mu + (M+\mu) \mathbb{P}(G^c) \nonumber \\
	\leq &  c + \nu-\mu + (M+\mu) \times \bigg(\bigg\lceil\frac{\lambda M}{\mu-c}\bigg\rceil\frac{\exp\left(-2\frac{(\mu-c)^2\frac{M}{c}}{\kappa^2}\right)}{1-\exp\left(-2\frac{(\mu-c)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}+\exp\left(-2\frac{(\lambda-1)^2M(\mu-c)}{\lambda  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)\bigg). \label{eq:finalBound}
	\end{align}
	We optimize over $\lambda>1$ to get the tightest possible bound. By Lemma \ref{lemma:optimal_causal} and \eqref{eq:finalBound}, we have the result for RR. 
	
	
	
	
	Next, we consider the case when $\mu < c$. We define the following events
	
	$F_{t_1,t_2}: \displaystyle\sum_{l=t_1}^{t_2} \underbar{$X$}_l \geq \displaystyle\sum_{l=t_1}^{t_2} R_l+M$, $F^{\tau}=\displaystyle\bigcup_{t_1=1}^{\tau} F_{t_1,\tau}$, $F_{t-1}=\displaystyle\bigcup_{\tau=t-\lceil\frac{\lambda M}{c-\mu}\rceil}^{t-1} F^{\tau}$, $F_{t}=\displaystyle\bigcup_{\tau=t-\lceil\frac{\lambda M}{c-\mu}\rceil+1}^{t} F^{\tau}$,                             $E: \displaystyle\sum_{l=t-\frac{\lambda M}{c-\mu}}^{t-1} \underbar{$X$}_l+M < \displaystyle\sum_{l=t-\frac{\lambda M}{c-\mu}}^{t-1} R_l$.\\
	
	By Lemma \ref{lem:Hoeffding}, it follows that  $\mathbb{P}(F_{t_1,t_2})\leq \exp\left(-2\frac{(c-\mu)^2 (t_2-t_1+1)}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right),$ and therefore, 
	\begin{align}
	\mathbb{P}(F^{\tau})&\leq \displaystyle \sum_{t_1=1}^{\tau-\lceil\frac{M}{\kappa-c}\rceil+1} \exp\left(-2\frac{(c-\mu)^2 (\tau-t_1+1)}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)\leq \frac{\exp\left(-2\frac{(c-\mu)^2 \frac{M}{\kappa-c}}{\kappa^2}\right)}{1-\exp\left(-2\frac{(c-\mu)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}. \label{eq:F_tau}
	\end{align}
	Using \eqref{eq:F_tau} and the union bound, $\mathbb{P}(F_{t})$ and $\mathbb{P}(F_{t-1})$ are upper bounded by
	\begin{equation}
	\bigg\lceil\frac{\lambda M}{c-\mu}\bigg\rceil \frac{\exp\left(-2\frac{(c-\mu)^2 \frac{M}{\kappa-c}}{\kappa^2}\right)}{1-\exp\left(-2\frac{(c-\mu)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}. \label{eq:F2}
	\end{equation}
	By Lemma \ref{lem:Hoeffding},  
	\begin{align}
	\mathbb{P}(E^c)&\leq \exp\left(-2\frac{((c-\mu)\lceil\frac{\lambda M}{c-\mu}\rceil-M)^2}{\frac{\lambda M}{c-\mu}  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right) \leq \exp\left(-2\frac{(\lambda-1)^2(c-\mu)M}{\lambda  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right). \label{eq:E2}
	\end{align} 
	By \eqref{eq:F2} and \eqref{eq:E2},
	\begin{align}
	\mathbb{P}(F^c_t \cap F^c_{t-1} &\cap E)\geq 1- \exp\left(-2\frac{(\lambda-1)^2(c-\mu)M}{\lambda  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)-2\bigg\lceil\frac{\lambda M}{c-\mu}\bigg\rceil \frac{\exp\left(-2\frac{(c-\mu)^2 \frac{M}{\kappa-c}}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}{1-\exp\left(-2\frac{(c-\mu)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}.
    \label{eq:FcapE2}
	\end{align}
	Consider the event $G = F^c_t \cap F^c_{t-1} \cap E$ and the following three cases. 
	%\begin{itemize}
	%	\item[--] 
	
	Case 1: The service is not hosted  at the edge during time-slot $t -\big\lceil\frac{\lambda M}{c-\mu}\big\rceil$: Conditioned on $F^c$, by the properties of the RR  policy, the service is not fetched in time-slots $t - \big\lceil\frac{\lambda M}{c-\mu}\big\rceil$ to $t-1$. It follows that in this case, the service is not  hosted  at the edge during time-slot $t$.
	%	\item[--] 
	
	Case 2: The service is hosted  at the edge during time-slot $t - \big\lceil\frac{\lambda M}{c-\mu}\big\rceil$ and is evicted in time-slot $\tilde{\tau}$ such that $t - \big\lceil\frac{\lambda M}{c-\mu}\big\rceil + 1 \leq \tilde{\tau} \leq t-2$: Conditioned on $F^c$, by the properties of the RR policy, the service is not fetched in time-slots $\tilde{\tau}+1$ to $t-1$. It follows that in this case, the service is not  hosted  at the edge during time-slot $t$.
	
	%\item[--] 
	
	Case 3: The service is hosted  at the edge during time-slot $t - \big\lceil\frac{\lambda M}{c-\mu}\big\rceil$ and is not evicted in time-slots $t - \big\lceil\frac{\lambda M}{c-\mu}\big\rceil + 1$ to $t-2$: In this case, in time-slot $t-1$, $t_{\text{evict}} \leq t - \big\lceil\frac{\lambda M}{c-\mu}\big\rceil$. Conditioned on $E$, by the properties of the RR  policy, condition in Step 16 in Algorithm \ref{algo:RR}  is satisfied for $\tau = t - \big\lceil\frac{\lambda M}{\mu-c}\big\rceil$.  It follows that in this case, the service is evicted in time-slot $t-1$ and therefore, the service is not hosted  at the edge in time-slot $t$.
	%\end{itemize}
	
	We thus conclude that conditioned on $F^c_{t-1} \cap E$, the service is not  hosted  at the edge during time-slot $t$. In addition, conditioned on $F^c_{t}$, the service is not fetched in time-slot $t$. 
	We now compute the expected cost incurred by the RR policy. By definition, 
	$
	\mathbb{E}[C_t^{\text{RR}}] =  \mathbb{E}[C_t^{\text{RR}}|G] \mathbb{P}(G) + \mathbb{E}[C_t^{\text{RR}}|G^c] \times \mathbb{P}(G^c).
	$
	Note that, 
	$
	\mathbb{E}[C_t^{\text{RR}}|G] = \nu, \  \mathbb{E}[C_t^{\text{RR}}|G^c] \leq c+ \nu + M.
	$
	Therefore,
	\begin{align}
	\mathbb{E}&[C_t^{\text{RR}}] = \nu + (c+M) \mathbb{P}(G^c) \leq  \nu + \exp\left(-2\frac{(\lambda-1)^2(c-\mu)M}{\lambda  (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)+ (c+M) \times \bigg\lceil\frac{2\lambda M}{c-\mu}\bigg\rceil \frac{\exp\left(-2\frac{(c-\mu)^2 \frac{M}{\kappa-c}}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}{1-\exp\left(-2\frac{(c-\mu)^2}{ (\kappa+c_{\text{max}}-c_{\text{min}})^2}\right)}. 
 \label{eq:finalBound2}
	\end{align}
	We optimize over $\lambda>1$ to get the tightest possible bound. By Lemma \ref{lemma:optimal_causal} and \eqref{eq:finalBound2}, we have the result for RR.  
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:RR_stochastic_theorem}]
	Follows by Lemma \ref{lemma:optimal_causal}, \eqref{eq:finalBound}, \eqref{eq:finalBound2}, the definition of $\sigma^{\mathcal{P}}$ in \eqref{eq:efficiencyRatio}, and the fact that the cost incurred in a time-slot by any policy is upper bounded by $M+c+\nu$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem \ref{thm:fixed_TTL}}
\begin{proof}
	Throughout this proof we consider  a renting cost sequence where the cost of renting is $c_{\text{max}}$ in each time-slot.
	
	Consider the case where $\kappa < M+c_{\text{max}}$. For this setting we construct a request sequence where a request arrives in the first time-slot and no requests arrive thereafter. OPT-OFF does not fetch the service and the total cost of service per request for this request sequence under OPT-OFF is one unit. Let $C^{\text{TTL}}$ be the cost of service per request for this request sequence under  TTL. TTL fetches the service on a request arrival and stores it on local edge server for $L$ time slots. Thus the cost of service incurred by TTL per request is $C^{\text{TTL}}=1+M+Lc_{\text{max}}.$ Therefore, $\rho^{\text{ TTL}}\geq 1+M+Lc_{\text{max}}.$	
	Next, we consider the case where $\kappa \geq M+c_{\text{max}}$ and $Lc_{\text{max}} > M$. For this setting we construct a request sequence where $\kappa$ requests arrive in the first time-slot and no requests arrive thereafter. In this case, $C^{\text{TTL}} = \kappa + Lc_{\text{max}} + M$. Consider an alternative policy which fetches the service before the first time-slot and hosts  it for one time-slot. The total cost of service for this policy is $M+c_{\text{max}}$. It follows that $\rho^{\text{TTL}}\geq \dfrac{\kappa+M+Lc_{\text{max}}}{M+c_{\text{max}}}.$
	Next, we consider the case where $\kappa \geq M+c_{\text{max}}$ and $Lc_{\text{max}} \leq M$. For this setting we construct a request sequence where $\kappa$ requests arrive in time-slots $1, L+2, 2L+3, \cdots, (u-1)L+u$ and no requests arrive in the remaining time-slots. In this case, $C^{\text{ TTL}} = u(\kappa + Lc_{\text{max}} + M)$. Consider an alternative policy which fetches the service before the first time-slot and hosts  it till time-slot $(u-1)L+u$. The total cost of service for this policy is $M+((u-1)L+u)c_{\text{max}}$. It follows that $$\rho^{\text{TTL}}\geq \sup_{u \geq 1} \dfrac{u(\kappa + Lc_{\text{max}} + M)}{M+((u-1)L+u)c_{\text{max}}} = \dfrac{\kappa + Lc_{\text{max}} + M}{Lc_{\text{max}}+c_{\text{max}}}.$$
%	\noindent The result follows from the three cases. 
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:TTL_stochastic_theorem}}
\begin{proof}[Proof of Lemma \ref{lemma:TTLstochastic}]
	We compute the expectation of the cost incurred by the TTL policy in time-slot $t$. Let $G$ be the event that there are no arrivals in time-slots $\max\{t-L,1\}$ to $t-1$. Under Assumption \ref{assum_stochastic}, 
	$\mathbb{P}(G) = p_0^{\min\{L,t-1\}}.$
	For the TTL policy, conditioned on $G$, the service is not hosted  at the beginning of time-slot $t$ and all requests received in time-slot $t$ are forwarded to the back-end server. In addition, the service is fetched if at least one request is received in time-slot $t$. It follows that $\mathbb{E}[C_t^{\text{TTL}}]  = M(1-p_0) + \nu.$
	If the service is hosted at the edge in time-slot $t$, the TTL policy pays a rent cost of $R_t$ and up to $\kappa$ results are served at the edge. The remaining requests are forwarded to the back-end server. It follows that
	$
	\mathbb{E}[C_t^{\text{TTL}}|G^c]  = \mathbb{E}[R_t] + \mathbb{E}[X_t-\min\{X_t,\kappa\}]= c + \nu- \mu.
	$
	Note that $\mathbb{E}[C_t^{\text{TTL}}] = \mathbb{E}[C_t^{\text{TTL}}|G] \mathbb{P}(G) + \mathbb{E}[C_t^{\text{TTL}}|G^c] \mathbb{P}(G^c)=(M(1-p_0)+\nu) p_0^{\min\{L,t-1\}} + (c + \nu-\mu) (1-p_0^{\min\{L,t-1\}}). $
	Moreover, $\mathbb{E}[C_t^{\text{OPT-OFF}}] \leq \nu.$
	It follows that $\Delta^{\text{TTL}} \geq M(1-p_0)p_0^{\min\{L,t-1\}} + (c-\mu)(1-p_0^{\min\{L,t-1\}}),$
	thus proving the result.
\end{proof}
%%
\begin{proof}[Proof of Theorem \ref{thm:TTL_stochastic_theorem}]
	Follows by Lemma \ref{lemma:TTLstochastic} and the fact that the cost per time-slot incurred by the optimal online policy is at most $\nu$.
\end{proof}

==> simulation_results_adv <==
\label{sec:simulation}
In this section, we present our simulation results  for Model \ref{model:partial}.  In addition to plotting the performance of $\alpha$-OPT, $\alpha$-RetroRenting, and the lower bound on the performance of any  online policy ($\alpha$-LB), we also simulate two policies which do not use partial hosting. We refer to the the offline optimal policy without partial hosting as OPT. The other policy called RetroRenting (RR) was proposed in \cite{narayana2021renting}. RR works on the same principle as that of  $\alpha$-RetroRenting without using partial hosting. We also plot the lower bound on the performance of any online policy which is not allowed to partially host the service (LB). The parameters used for each data point in a plot are given in the figure caption.  Although our analysis for Model 1 holds under Assumption \ref{assum_one_request} and for adversarial arrival processes, in this section, we consider more general arrival processes with more  than one request per time-slot. We also consider the setting where request arrivals are stochastic. 
%The corresponding results for Model \ref{model:random} are qualitatively similar.
\subsection{Synthetic Request Arrivals and Rent Costs}

The first set of results use synthetic request arrival and rent cost sequences. Unless stated otherwise, the request arrival process is i.i.d. Bernoulli with parameter $p$. We model the time-varying rent cost sequence using the Autoregressive moving-average (ARMA) model \cite{box2011time}, specifically, ARMA(4,2). To choose the parameters of the model, we fit the model to real world price data obtained from \cite{awsprices}, which provides region-wise prices of unused EC2 capacity in the Amazon Web Services (AWS) cloud.
%\color{red} To model the time-varying rent cost sequence with a given mean value $c$, we use the Autoregressive moving-average (ARMA) model \cite{box2011time}. Specifically, we use the ARMA(4,2) model, with parameters chosen by fitting the model to real world price data obtained from \cite{awsprices}, which consists of the region-wise prices of unused EC2 capacity in the Amazon Web Services (AWS) cloud.  \color{black} 


%%%%%%%%%%%%%%%%%%%% PLOTS (SET 1)%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/1_submit_2.eps}
	
	\caption{Total cost per time slot as a function of $\alpha+g(\alpha)$ for $M = 10$, $c = 0.35$, $p=0.35$, and $\alpha=0.4$}
		\label{fig:1}
	\end{center}

\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% HISTOGRAMS %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \begin{figure}[tbh]
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/middle0_submit.eps}
		\caption{Number of time-slots per hosting state under $\alpha$-RR as function of $\alpha+g(\alpha)$ for $M = 10$, $c = 0.35$, $p=0.35$, and $\alpha=0.4$ }\label{fig:middle0}
	\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/4_submit.eps}
		\caption{Total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha+g(\alpha)<1$. Here $c=0.35$, $\alpha=0.239$, $g(\alpha)=0.380$ and $p=0.42$ }
		\label{fig:4}
	\end{center}
\end{figure}



\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/7_submit.eps}
		\caption{Total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha+g(\alpha) \geq 1$. Here $c=0.35$, $\alpha=0.5$, $g(\alpha)=0.7$ and $p =0.42 $}\label{fig:7}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/16_submit.eps}
		\caption{Total cost per time slot as a function of request arrival probability ($p$) for the case when $\alpha +g(\alpha)<1$. Here $c=0.35$, $M = 10$, $\alpha=0.239$, $g(\alpha)=0.38$}\label{fig:16}
	\end{center}
\end{figure}
         \begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/17_submit.eps}
		\caption{Total cost per time slot as a function of request arrival probability ($p$) for the case when $\alpha +g(\alpha)\geq1$. Here $c=0.35$, $M = 10$, $\alpha=0.5$, $g(\alpha)=0.7$}\label{fig:17}
	\end{center}
\end{figure}
 
 %%%%%%%%%%%%%% markov %%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/GE1_submit.eps}
	 	\caption{Total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha=0.3$, $g(\alpha)=0.4$, $\alpha_1 = 0.4$, $g(\alpha_1) = 0.3$, $\alpha_2 = 0.5$, $g(\alpha_2) = 0.15$ and $c = 0.5$}
	 	\label{fig:GE1}
	\end{center}
	
\end{figure}
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set1/GE2_submit.eps}
		\caption{Hosting Status over time for different policies for the case when $\alpha=0.3$, $g(\alpha)=0.4$, $\alpha_1 = 0.4$, $g(\alpha_1) = 0.3$, $\alpha_2 = 0.5$, $g(\alpha_2) = 0.15$ and $c = 0.5$}
			\label{fig:GE2}
	\end{center}

\end{figure}



In Figure \ref{fig:1}, we plot the total cost per time-slot incurred by various policies as a function of $\alpha + g(\alpha)$. We see that the performance gap between policies that are allowed to use partial hosting ($\alpha$-RetroRenting/$\alpha$-OPT/$\alpha$-LB) and their counterparts that are not allowed to use partial hosting (RetroRenting/OPT/LB) is significant for $\alpha + g(\alpha) < 1$ and vanishes for $\alpha + g(\alpha)\geq 1$. 

In Figure \ref{fig:middle0}, we illustrate the number of time-slots for which the $\alpha$-RetroRenting uses the three possible hosting levels as a function of $\alpha + g(\alpha)$ over a time-horizon of 10000 time-slots. As expected, $\alpha$-RetroRenting does not use partial hosting for $\alpha + g(\alpha) \geq 1$.

In Figures \ref{fig:4}, \ref{fig:7}, \ref{fig:16}, and \ref{fig:17}, we plot the total cost per time-slot incurred by various policies as a function of the fetch cost $M$ and request arrival probability $p$, for two cases, namely, $\alpha + g(\alpha) < 1$ and $\alpha + g(\alpha) \geq 1$. We observe a performance gap between policies that are allowed to use partial hosting ($\alpha$-RetroRenting/$\alpha$-OPT/$\alpha$-LB) and their counterparts that are not allowed to use partial hosting (RetroRenting/OPT/LB) only if $\alpha + g(\alpha) < 1$.

In the next set of results presented in Figures \ref{fig:GE1} and \ref{fig:GE2}, we compare the performance of RR and $\alpha$-RetroRenting with a third policy call multiple--RR which works on the same principle as $\alpha$-RetroRenting/RetroRenting and is allowed to use two additional intermediate hosting levels ($\alpha$, $\alpha_1$, $\alpha_2$). For this set of results, we use the Gilbert-Elliot model \cite{liu2010indexability} \color{black} for the request arrival process. The parameters of the model are as shown in Figure \ref{fig:gilbert}. The request arrival process is Bernoulli(0.9) when the Markov chain is in state 0, and Bernoulli(0.1) otherwise.  \color{black} 


 \begin{figure}[h] 
		\begin{center}
			\begin{tikzpicture}[font=\sffamily]
			\usetikzlibrary{calc,arrows.meta,positioning}
			% Setup the style for the states
			\tikzset{node style/.style={circle,draw=black!90,thick, 
					minimum width=.4cm,
					line width=.2mm,
					fill=white!20}}
			%dn-dummynode, o1-one_1, t1-two_one, th_1-three_1
			% Draw the states
			\node[node style] at (6, 1)     (o1)     {\tiny{0}};
			\node[node style] at (9, 1)     (o2)     {\tiny{1}};
			
			\draw[every loop,
			auto=right,
			line width=0.2mm,
			>=latex,
			draw=black,
			fill=black]
		
			(o1)     edge[ bend left=40, auto=left] node {$0.01$} (o2)
			(o1)     edge[loop above] node {$0.99$} (o1)
			(o2)     edge[loop above] node {$0.99$} (o2)
			(o2)     edge[bend left=40, auto=left] node {$0.01$} (o1);
			
			
			
			\end{tikzpicture}
			\caption{The Gilbert-Elliot model}
			\vspace{15pt}
			\label{fig:gilbert}
		\end{center}
\end{figure}

 
In Figure \ref{fig:GE1}, we see that the additional intermediate hosting options available to multiple--RR brings down the cost incurred. 
In Figure \ref{fig:GE2}, we plot the hosting status $r_t$ for the three different policies as a function of time.

%%% table %%%
\begin{comment}

\begin{table}
  \centering
  \begin{tabular}{ | m{1cm} | m{1cm}| m{1cm} | m{1cm}| m{1cm} | m{1cm} | } 
    \hline
    $\alpha$ & 0 & 0.3 & 0.4 & 0.5 & 1 \\ 
    \hline
    $g(\alpha)$ & 1 & 0.5 & 0.4 & 0.15 & 0 \\ 
    \hline
  \end{tabular}
  \caption{Multiple cache levels} \label{tab:multiple-levels}
\end{table}
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% PLOTS (SET 2) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Trace-driven Simulations}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set2/j2_4_submit.eps}
		\caption{Total cost per time slot for as a function of fetch cost ($M$) for the case when $\alpha+g(\alpha)<1$. Here $c=0.135$, $\alpha=0.239$, $g(\alpha)=0.38$ }\label{fig:j2_4}
	\end{center}
\end{figure}
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set2/j2_7_submit.eps}
		\caption{Total cost per time slot for as a function of fetch cost ($M$) for the case when $\alpha+g(\alpha) \geq 1$. Here $c=0.135$,  $\alpha=0.5$, $g(\alpha)=0.7$}\label{fig:j2_7}
	\end{center}
\end{figure}

For the next set of results, 
For the next set of results, we use trace-data obtained from a Google Cluster \cite{googlecluster} for the arrival process and time-varying spot prices of spare server capacity in the  AWS cloud as given in \cite{awsprices} as the rent cost.
%we use trace-data obtained from a Google Cluster \cite{googlecluster} for the arrival process. We use a time-slot duration small enough to ensure that there is at most one request in a time-slot. This trace-data has requests for four types of jobs/services identified as ``Job 0", ``Job 1", ``Job 2", and ``Job 3". In this section, we present results for ``Job 2" (Figures \ref{fig:j2_4}, \ref{fig:j2_7}). We use time-varying rent cost obtained from real world data. Specifically, we use the time-varying spot prices of spare server capacity in the  AWS cloud as given in \cite{awsprices}. This data \cite{awsprices} consists of details like current spot price for different instances for different regions. We use the spot price details of Canada region for one instance 'm4.large'. We normalise this data by dividing each entry by average value of spot prices. \color{black}

%In Figure \ref{fig:j2_1}, we plot the total cost per time-slot incurred by various policies as a function of $\alpha + g(\alpha)$. We see that the performance gap between policies that are allowed to use partial hosting ($\alpha$-RetroRenting/$\alpha$-OPT) and their counterparts that are not allowed to use partial hosting (RetroRenting/OPT) is significant for $\alpha + g(\alpha) < 1$ and vanishes for $\alpha + g(\alpha)\geq 1$. 

In Figures \ref{fig:j2_4} and \ref{fig:j2_7}, we plot the total cost per time-slot incurred by various policies as a function of the fetch cost $M$ for the case when $\alpha + g(\alpha) < 1$ and $\alpha + g(\alpha) \geq 1$ respectively. As expected, we observe a performance gap between policies that are allowed to use partial hosting ($\alpha$-RetroRenting/$\alpha$-OPT) and their counterparts that are not allowed to use partial hosting (RetroRenting/OPT) only in the first case.  

\begin{comment}
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set2/j2_1_submit.eps}
	
	\caption{Total cost per time slot for Job2 data as a function of $\alpha+g(\alpha)$ for $M = 10$, $c = 0.135$, $\alpha$=0.4}\label{fig:j2_1}
	\end{center}
	
\end{figure}
\end{comment}



\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% PLOTS (SET 3) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Simulations on GPS Trajectory Dataset}
In this set of simulations, we used GPS trajectory dataset\cite{zheng2008understanding}\cite{zheng2009mining}\cite{zheng2010geolife} which was collected as a part of Geolife Project by Microsoft Research Asia. For each trajectory, we extract its start and end locations as the source and target of a shortest path query, respectively. So each query is a request to find the shortest distance from source to destination. \\
To find the shortest path, we used Road Network data of Beijing city. Using Djikstra's shortest path algorithm we generated sequence of nodes corresponding to shortest path for each query.\\
Then, we used a greedy algorithm, namely, fractional knapsack to sort paths having maximum importance which is defined as ratio of number of queries it can answer to the length of that path.\\
Given, all these and a cache storage, we now put all those paths in order of importance to fill the cache.\\
Each query has a timestamp and is collected over five years from 2007-12. We used the first three years query for training purpose and the last two years for testing to see if the cache generated from training is able to serve the unseen queries.\\
Below \ref{fig:789}, shows the graph of stored cache percentage vs the percentage of test queries answered.
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set3/789.eps}
		\caption{}\label{fig:789}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set3/costVsAlpha.eps}
		\caption{}\label{fig:costvsalpha}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set3/costVsM.eps}
		\caption{}\label{fig:costvsm}
	\end{center}
\end{figure}

\end{comment}





==> simulation_results_stochastic <==
\label{sec:simulation}
\color{black}
In this section, we present our simulation results for Model $2$. In addition to $\alpha$-RR, we also simulate a policy called RetroRenting (RR) which was proposed in \cite{narayana2021renting} and does not use partial hosting. RR works on the same principles as that of  $\alpha$-RR without using partial hosting. \color{violet} Although our analysis for Model 2 holds under Assumption \ref{assum_one_request} and stochastic arrivals, in this section, we consider more general arrival
processes with more than one request per time-slot. We also use trace-based arrivals to compare the performance of various policies. \color{black}

\color{black}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% Plots (stochastic case) 8 plots%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Synthetic Request Arrivals and Rent Costs}
We consider two types of synthetic request arrivals, namely, Poisson and Markovian. We model the time-varying rent cost sequence for both kinds of arrivals using the Autoregressive moving-average (ARMA) model \cite{box2011time}, specifically ARMA(4,2) with expected rent cost in a slot given as $c$. To choose the parameters of the model, we fit the model using the process described in \cite{Narayana2021OnlinePS} to real world price data obtained from \cite{awsprices}, which provides region-wise prices of unused EC2 capacity in the Amazon Web Services (AWS) cloud.
\subsubsection{Poisson Request Arrivals}
The first set of results are for i.i.d. Poisson request arrivals with parameter $\lambda$ over 10,000 time slots. We use synthetic values for the available partial storage size $\alpha$ and corresponding forwarding cost $g(\alpha)$ for this first set of simulations, as given in the figure captions. In addition to $\alpha$-RR and RR, we also plot the lower bound on the performance of any deterministic online policy ($\alpha$-LB) and a lower bound on the performance of any deterministic online policy which is not allowed to partially host the service (LB). The expressions for these lower bounds can be found in \cite[Lemma 14]{RRtompecs} and Lemma \ref{lemma:optimal_causal} in the appendix respectively. 
\begin{comment}
synthetic request arrival and rent cost sequences. Unless stated otherwise, the request arrival process is
\end{comment}


\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{tompecsfigures/tompecs_fig12.eps}
		\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $c=4.5$, $\alpha=0.30$, $g(\alpha)=0.50$, and $\lambda=2$ }
		\label{fig:b1}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{poissonPlots/poisson_M_mid.eps}
		\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $c=4.5$, $\alpha=0.30$, $g(\alpha)=0.50$, and $\lambda=4$ }
		\label{fig:b3}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{poissonPlots/fig14_updated.eps}
		\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $c=4.5$, $\alpha=0.30$, $g(\alpha)=0.50$, and $\lambda=8$ }
		\label{fig:b5}
	\end{center}
\end{figure}

In Figures \ref{fig:b1}-\ref{fig:b5}, we first plot the histogram of hosting status and then the total cost per time slot under the two policies as a function of the fetch cost ($M$), for different values of request arrival intensity ($\lambda$). 

% From first two plots of Figure \ref{fig:b1}, we observe that for very low values of fetch cost $M$, $\alpha$-RR either hosts $\alpha$ fraction of the service or does not host it at all. For higher values of $M$, $\alpha$-RR and RR do not host the service. Overall both policies lean towards not hosting the service as the average number of arrivals per time-slot is smaller than the rent cost and thus it is cost effective to serve requests via the cloud instead of incurring rent cost. 
From the first two plots of Figure \ref{fig:b1}, we observe that RR does not host the service at all, while $\alpha$-RR also does the same except when $M$ is very small when it uses partial storage, albeit very rarely. Both policies lean towards not hosting the service as the average number of arrivals per time-slot $\lambda$ is smaller than the average rent cost $c$ here, and thus it is cost effective to serve requests via the cloud instead of incurring rent cost. Here, the lower bounds of online policies, namely, LB and $\alpha$-LB, coincide with each other. Also, as $M$ increases, the performance of RR and $\alpha$-RR approaches the lower bound.
%Since the average number of request per time slot given by $\lambda=2$ is much less compared to the average rent cost considered (i.e., $c=4.5$), both the policy finds forwarding the request to be beneficial than storing anything at all.
%This is explained by the fact that as $p$ is very less here, it becomes optimal to forward any request to the edge server than to host $\alpha$ fraction or the entire service.
%The variation in cost of both these policies is confirmed from the third plot, where after some value of $M$ (here $M=60$) both the policies converge.
In Figure \ref{fig:b3}, we note that the average number of requests and average rent cost is comparable, and here $\alpha$-RR hosts $\alpha$ fraction of the service at all times while RR hosts the entire service. We note that $\alpha$-RR outperforms RR for smaller values of $M$, while they have similar costs for larger values of $M$.
%The difference in cost is seen from the same figure, which explains renting $\alpha$ is the optimal thing to do in this case.
Figure \ref{fig:b5} considers a larger value of $\lambda$ where hosting the entire service is optimal, and here both the policies host the entire service at all times for all values of $M$ considered. {\color{red}Dynamic range of figure}\color{black}


\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{poissonPlots/poisson_c.eps}
		\caption{Histogram of hosting status \& total cost per time slot as a function of rent cost ($c$) for the case $M=40$, $\alpha=0.30$, $g(\alpha)=0.50$, and $\lambda=4$ }
		\label{fig:b7}
	\end{center}
\end{figure}



In Figure \ref{fig:b7}, we first plot the histogram of hosting status and then the total cost per time slot under the two policies as a function of the rent cost ($c$), for a fixed value of request arrival intensity ($\lambda$). 
%we plot the histogram of hosting status under the two policies as a function of the rent cost $c$ for a fixed value of request arrival probability $p$.
%% write here %%
% From Figure \ref{fig:b7}, we observe that initially $\alpha$-RR hosts $\alpha$ service at all times but gradually as rent cost $c$ increases it settles down to hosting none similar to RR which hosts entire service for very low $c$ and then stores none at all as we increase the rent cost.
From the first two plots in Figure \ref{fig:b7}, we observe that for low values of $c$, $\alpha$-RR and RR host the entire service in all time-slots. For $3\leq c \leq 7$, $\alpha$-RR hosts $\alpha$ fraction of the service for most of the time. For higher values of the rent cost ($c \geq 8$), $\alpha$-RR and RR both do not host the service. We note that $\alpha$-RR outperforms RR for values of $c$ close to average arrival rate ($\lambda$) and the performance of $\alpha$-RR and RR is comparable for low and large $c$. This is also consistent with what we observe in Figures \ref{fig:b1}-\ref{fig:b5}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% Plots(Markov chain) 12 plots %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Markovian Request Arrivals}

\begin{figure}[h] 
		\begin{center}
			\begin{tikzpicture}[font=\sffamily]
			\usetikzlibrary{calc,arrows.meta,positioning}
			% Setup the style for the states
			\tikzset{node style/.style={circle,draw=black!90,thick, 
					minimum width=.4cm,
					line width=.2mm,
					fill=white!20}}
			%dn-dummynode, o1-one_1, t1-two_one, th_1-three_1
			% Draw the states
			\node[node style] at (6, 1)     (o1)     {\tiny{H}};
			\node[node style] at (9, 1)     (o2)     {\tiny{L}};
			
			\draw[every loop,
			auto=right,
			line width=0.2mm,
			>=latex,
			draw=black,
			fill=black]
		
			(o1)     edge[ bend left=40, auto=left] node {${P}_{H\rightarrow L}$} (o2)
			(o1)     edge[loop left] node {$(1-{P}_{H\rightarrow L})$} (o1)
			(o2)     edge[loop right] node {$(1-{P}_{L\rightarrow H})$} (o2)
			(o2)     edge[bend left=40, auto=left] node {${P}_{L\rightarrow H}$} (o1);
			
			
			
			\end{tikzpicture}
			\caption{The Gilbert-Elliot model}
			\vspace{15pt}
			\label{fig:gilbert}
		\end{center}
\end{figure}

% \subsection{Markovian Arrivals}
\begin{comment}
In the next set of results, we compare the performance of RR and $\alpha$-RR with two optimal offline policies call Markov Decision Process (MDP) and Arrival Based Caching (ABC) \cite{ABC}. 
\end{comment}
For the next set of results, we use the Gilbert-Elliot model \cite{liu2010indexability} \color{black} for the request arrival process. The parameters of the model are as shown in Figure \ref{fig:gilbert}. The request arrival process is Poisson(200) when the Markov chain is in high state (\textit{H}), and Poisson(10) in the low state (\textit{L}). The values of partial storage $\alpha$ and forwarding cost $g(\alpha)$ used here are chosen based on a curve derived from a real dataset (see Figure \ref{fig:789}); details are presented in Section~\ref{derived galpha}. From Figure \ref{fig:789}, we see when $\alpha=0.16$, forward cost $g(0.16)$ is $0.76$ which is the minimum $\alpha + g(\alpha)$ pair among all pairs.

In the following series of experiments, we vary the transition probabilities for the request arrival process and compare the performance of various policies. We also compare the performance of RR and $\alpha$-RR with two other policies that know the statistics of the request arrivals and the expected rent cost $c$.

The first policy, referred to as the MDP policy, formulates the hosting problem as a Markov Decision Process. The second policy called Arrival Based Caching (ABC) proposed in \cite{ABC} makes hosting decisions based only on the request arrival rate in the current time-slot and the statistics of the arrival process. 

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{stochasticSimulationSet1/newset/c0404.eps}
	 	\caption{Histogram of hosting status \& total cost per time slot as a function of rent cost ($c$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $M = 50$ and ${P}_{H\rightarrow L} = 0.4$, ${P}_{L\rightarrow H} = 0.4$}
	 	\label{fig:m1}
	\end{center}
	
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{stochasticSimulationSet1/newset/M0404.eps}
	 	\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $c = 20$, and ${P}_{H\rightarrow L} = 0.4$, ${P}_{L\rightarrow H} = 0.4$}
	 	\label{fig:m3}
	\end{center}
\end{figure}

In the first three plots in Figure \ref{fig:m1}, we plot the histogram of the hosting status under the three policies as a function of the rent cost $c$. Here, the average number of requests per time slot is $105$ and transition probability ${P}_{H\rightarrow L}$ is same as ${P}_{L\rightarrow H}$ which is $0.4$. We observe that for low values of rent cost ($c \leq 20$), MDP hosts the entire service in all time-slots. For higher values of rent cost $20 < c \leq 150$, MDP hosts $\alpha$ fraction of the service in all time-slots. For $160 \leq c \leq 170$, MDP varies between hosting $\alpha$ fraction of the service and not hosting the service. For even higher values of rent cost ($c > 170$), MDP does not host the service. These trends are explained by the fact that as the expected rent cost $c$ increases, the cost incurred by serving requests via the cloud becomes lower than the cost of renting edge resources to host the service at the edge. The hosting status under $\alpha$-RR has a similar trend; however, the range of values of rent cost over which $\alpha$-RR hosts at least a part of the service is larger than MDP. RR hosts the entire service for low values of rent cost and does not host the service when rent cost $c$ is above a threshold, $c=80$. For intermediate values of rent cost, it varies between hosting the entire service and not hosting the service. As a consequence of the hosting status under the three policies, the total cost incurred under all three policies is very close for very low and very high values of rent cost. For rent costs, $c<180$, $\alpha$-RR outperforms RR and RR outperforms $\alpha$-RR for rent cost $c$ in the range $[180, 310]$.

Similarly, in the first three plots in Figure \ref{fig:m3}, we plot the histogram of hosting status under the three policies as a function of the fetch cost $M$. 
We observe that for most values of fetch cost $M$, MDP hosts $\alpha$ fraction of the service in all time-slots. 
%This trend is due to the fact that the rent cost is very less, so increasing fetch cost won't change the hosting status. 
Under $\alpha$-RR the hosting status varies between $\alpha$ fraction of the service and the entire service. We observe that $\alpha$-RR outperforms RR for low values of $M$ and their performance converges as $M$ increases. 

\begin{figure}
	\begin{center}
        \includegraphics[width=1\columnwidth]{tompecsfigures/tompecs_figure19.eps}
	 	\caption{Histogram of hosting status \& total cost per time slot as a function of rent cost ($c$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $M = 50$ and ${P}_{H\rightarrow L} = 0.2$, ${P}_{L\rightarrow H} = 0.1$}
	 	\label{fig:m5}
	\end{center}
\end{figure}

	
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{stochasticSimulationSet1/newset/fig20_updated2.eps}
	 	\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $c = 20$, and ${P}_{H\rightarrow L} = 0.2$, ${P}_{L\rightarrow H} = 0.1$}
	 	\label{fig:m7}
	\end{center}
\end{figure}

Unlike Figures~\ref{fig:m1} and \ref{fig:m3}, we next consider lower values of transition probabilities for the request arrival process, and again compare the performance of the three policies as a function of the rent cost $c$. For Figures \ref{fig:m5} and \ref{fig:m7}, the average number of requests per time slot is $73.33$ and transition probability ${P}_{H\rightarrow L}$ is $0.2$ whereas ${P}_{L\rightarrow H}$ is $0.1$. From Figure \ref{fig:m5}, we observe that $\alpha$-RR outperforms RR for most values of $c$. For very high values of $c$, the total cost incurred under all policies is close. We thus note that even though that MDP and ABC know the statistics of the arrival process while $\alpha$-RR does not have that information, the performance of $\alpha$-RR is comparable with MDP and ABC.  We note a similar trend in Figure \ref{fig:m7}, with RR performing poorly for all values of $M$ considered.


\begin{figure}
\centering
\parbox{7.3cm}{
\vspace{-0.3cm}
\includegraphics[width=7.3cm]{stochasticSimulationSet1/newset/c0801.eps}
\caption{Histogram of hosting status \& total cost per time slot as a function of rent cost ($c$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $M = 50$ and ${P}_{H\rightarrow L} = 0.8$, ${P}_{L\rightarrow H} = 0.1$}
\label{fig:m9}}
\quad
\begin{minipage}{7.3cm}
\includegraphics[width=7.3cm]{stochasticSimulationSet1/newset/M0801.eps}
\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $c = 20$, and ${P}_{H\rightarrow L} = 0.8$, ${P}_{L\rightarrow H} = 0.1$}
\label{fig:m11}
\end{minipage}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{stochasticSimulationSet1/newset/c0801.eps}
	 	\caption{Histogram of hosting status \& total cost per time slot as a function of rent cost ($c$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $M = 50$ and ${P}_{H\rightarrow L} = 0.8$, ${P}_{L\rightarrow H} = 0.1$}
	 	\label{fig:m9}
	\end{center}
	
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{stochasticSimulationSet1/newset/M0801.eps}
	 	\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha=0.16$, $g(\alpha)=0.76$, $\alpha_1 = 1$, $g(\alpha_1) = 0.6$, $c = 20$, and ${P}_{H\rightarrow L} = 0.8$, ${P}_{L\rightarrow H} = 0.1$}
	 	\label{fig:m11}
	\end{center}
	
\end{figure}
In the last set of  Figures \ref{fig:m9} and \ref{fig:m11},  we consider a request arrival process with very asymmetric transition probabilities. The average number of requests per time slot is $31.11$ and transition probability ${P}_{H\rightarrow L}$ is $0.8$ whereas ${P}_{L\rightarrow H}$ is $0.1$. Here, the underlying Markov chain spends most of its time in the low state.
Similar to previous experiments, from Figure \ref{fig:m9}, we conclude that for low values of rent cost $c$, $\alpha$-RR outperforms RR. For intermediate values of $c$, RR performs better than $\alpha$-RR  and for high values of $c$, the total cost incurred under all policies is close. For the same request arrival process, we plot the total cost vs $M$ in Figure \ref{fig:m11}, and find that $\alpha$-RR outperforms RR for all values of $M$ considered.

%%%% summary
% From figures \ref{fig:m1},\ref{fig:m5},\ref{fig:m9} we can summarize that as $c$ is less or comparable to average number of requests, the obvious choice for the $\alpha$-RR is to rent $\alpha$ rather that entire service.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% PLOTS (GPS trajectory data) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Simulations on GPS Trajectory Dataset}\label{derived galpha}
% \color{red}
In the next set of simulations, we use a real dataset to construct the forwarding cost function $g(\cdot)$ for a shortest path query system. In particular, we use a GPS trajectory dataset \cite{zheng2008understanding}\cite{zheng2009mining}\cite{zheng2010geolife} collected as a part of the Geolife Project by Microsoft Research Asia. This dataset contains 17,621 cab trajectories from Beijing, China, compiled over five years from 2007-12. Using this data, we model a service which when queried with a source-destination pair, returns the shortest path corresponding to that input. As before the goal is to host this service in the most cost-efficient way. Next, we describe how the edge cache size is measured and our algorithm to decide what goes in the cache.

The complete library at the server is considered to be of size $N \times P$ where $N$ is the total number of queries and $P$ is the total number of nodes in the shortest path corresponding to all $N$ queries. We host a fraction of this dataset in our locally available cache to assist with answering future queries. The cache size is measured by the total number of nodes stored across all the cached trajectories.

We extract each trajectory's start and end locations as the source and destination nodes of the shortest path query, respectively. So each query is a request to the system which returns the shortest distance from source to destination. To find the trajectory between each source-destination pair, we used Road Network data\cite{10.1145/2213836.2213872} of Beijing city. Using Dijkstra's shortest path algorithm\cite{10.1145/146585.146588}, we generated a sequence of nodes corresponding to the shortest path for each query.

We use the query data from the first three years of the GPS trajectory dataset \cite{zheng2008understanding}\cite{zheng2009mining}\cite{zheng2010geolife} to decide which paths should be hosted at the edge, given a certain cache size. We use a greedy strategy, namely the fractional knapsack\cite{fractionalknapsack} algorithm, and to enable this we sort all the paths according to their `normalized hit rate'. For any path hosted at the edge, we assume that it will result in a `hit' whenever a query has both its source and destination nodes on the path. Then, the normalized hit rate for a path is defined as the ratio of the number of hits to the total count of nodes forming that path. A path with high normalized hit rate can serve more queries per unit used cache size, if hosted at the edge. Finally, given any cache size, the fractional knapsack algorithm chooses to greedily host paths with the highest normalized hit rates. 
%Our cache exploits the optimal subpath property(see Lemma 1 in \cite{10.1145/2213836.2213872}), which allows a cached shortest path to answer any query with source and destination nodes on the path. 
%%%%%%%%%%%%%%%%%%
%\color{black}

%A GPS trajectory of this dataset is represented by a sequence of time-stamped points in a period of over four years. We used the query data of first three years  for training purpose (to fill cache). 
Next, for any given cache size and the corresponding subset of paths hosted at the edge as describe above, we use the query data of the fourth year from the GPS trajectory dataset to estimate the fraction of queries that can be answered at the edge. Figure \ref{fig:789} plots the fraction of test queries served by the edge cache vs the available cache size. Here, we represent the cache size as a fraction, defined as the ratio of the number of nodes corresponding to the cached paths and the total number of nodes involved in all paths that appear in the first three years of the GPS trajectory dataset. For any fraction $\alpha$, the value on the curve\footnote{Note that the fraction of queries answered is less than $1$ even when the cache size is large enough to store all the paths. This is because the cache content is decided based on queries from the first three years, whereas the fraction of queries answered is decided based on the data from the fourth year wherein new paths were queried whose source-destination pairs did not lie on any of the previously seen paths.} is used as a proxy for $1-g(\alpha)$. More details about the above procedure are available in \cite{GpsRoadNetworkAnalysis}.
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{set3/fif23_updated.eps}
		\caption{Percentage of queries answered by the fraction of cache stored at the edge}\label{fig:789}
	\end{center}
\end{figure}

We now compare the performance of RR and $\alpha$-RR policies on the queries from the fourth year of the GPS trajectory dataset. In Figure \ref{fig:costvsalpha}, we plot the total cost of all requests as a function of cache capacity $\alpha$ with $c = 0.4$. We observe that the cost for $\alpha$-RR is minimum when $\alpha$ is 0.5.
\begin{figure}
	\begin{center}
% 		\includegraphics[width=1\columnwidth]{set3/mapdata_alpha.eps}
\includegraphics[width=1\columnwidth]{set3/costVsALPHA.eps}
		\caption{Total cost of all requests as a function of cache stored when $c = 0.4$}\label{fig:costvsalpha}
	\end{center}
\end{figure}
We use this cache size and rent cost $c = 0.4$ in Figure \ref{fig:costvsm}, where we plot the total cost per time slot as a function of fetch cost ($M$). We observe that $\alpha$-RR performs much better than RR, thus highlighting the potential cost benefits that can be derived by efficiently utilizing partial storage. Moreover, it even outperforms offline optimal policy without partial storage (OPT).

% {\color{red} Are there other policies we can compare with for this dataset? What about offline optimal?\color{black}}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{stochasticSimulationSet1/newset/m3.eps}
		\caption{Histogram of hosting status \& total cost per time slot as a function of fetch cost ($M$) for the case when $\alpha = 0.5$ and $c = 0.4$}\label{fig:costvsm}
	\end{center}
x\end{figure}
